Compile-Time Tensor Shape Checking via Staged Shape-Dependent Types

When writing programs involving matrices or tensors in general, it is desirable to rule out the inconsistency of tensor shapes (i.e., the generalization of matrix sizes) before actual computation. For this purpose, some languages provide dependent types such as Mat m n, and others offer refinement types to track predicates for shapes. Despite the theoretical maturity, however, such methods are often unhandy for continuous software development due to the requirement of proofs for judging type equality or subtyping; even automated proving is often unsuitable due to its unforeseeable time consumption. To remedy this, our study provides an alternative formalization by using staging. Based on the observation that conditions for the shape consistency can be extracted before running the actual tensor computations in many typical cases, we ensure such consistency by assertions evaluated as compile-time computations, not by proofs. Under this formalization, we can verify the consistency virtually statically in the sense that inconsistencies as to tensor shapes will be immediately detected as assertion failures during compile-time computation. Our work achieves a mathematical guarantee that successfully generated code is always consistent with respect to tensor shapes. Furthermore, to vastly lessen the burden of adding shape- or stage-related descriptions, we (1) allow shape-related arguments to be implicit and infer them in a best-effort manner, and (2) offer a non-staged surface language that seemingly resembles ordinary dependently-typed languages and translate its programs into the staged core language. By a prototype implementation, we confirm that our language is expressive enough to verify a number of programs, including several examples offered by ocaml-torch.

==> proglangtools/progbnf.tex <==
\makeatletter
  \def\progbnf@unique{\progbnf@unique@dummy}
  \def\progbnf@car#1#2\progbnf@end{#1}
  \def\progbnf@cdr#1#2\progbnf@end{#2}
  \def\local@then#1\else#2\fi{\fi#1}
  \def\local@hop#1\fi{\fi#1}
  \def\progbnf@tab{&}
  \def\progbnf@break{\\}
  \newcommand\bnfeq{\ \mathrel{::=}\ }
  \newcommand\bnfsep{\ \mid\ }
  \newcommand\bnf[3][]{%
    % #1 : the set defined by the metavariable (if non-empty)
    % #2 : the metavariable to be defined
    % #3 : the `|`-separated constructs
    \ifx\progbnf@unique#1\progbnf@unique\else#1\ni\fi
    #2\progbnf@tab\bnfeq\progbnf@iter#3|\progbnf@end
  }
  \newcommand\bnfnotab[3][]{%
    % #1 : the set defined by the metavariable (if non-empty)
    % #2 : the metavariable to be defined
    % #3 : the `|`-separated constructs
    \ifx\progbnf@unique#1\progbnf@unique\else#1\ni\fi
    #2\bnfeq\progbnf@iter#3|\progbnf@end
  }
  \def\progbnf@iter#1|#2\progbnf@end{%
    % #1 : the first construct
    % #2 : the rest of the constructs
    % If #2 starts with `*`, then a line break is inserted before #2.
    {#1}% Encloses #1 so that #1 does not expand the next `\ifx`
    \ifx\progbnf@unique#2\progbnf@unique\else\local@hop
      \progbnf@rest{#2}%
    \fi
  }
  \def\progbnf@rest#1{%
    % #1 : the rest of the constructs
    \expandafter\if\expandafter*\progbnf@car#1\progbnf@end
    \local@then
      \progbnf@break\progbnf@tab\phantom{\bnfeq}\hspace{-1em}%
        \bnfsep\expandafter\progbnf@iter\progbnf@cdr#1\progbnf@end\progbnf@end
    \else\local@hop
      \bnfsep\progbnf@iter#1\progbnf@end
    \fi
  }
\makeatother


==> proglangtools/progindent.tex <==
\makeatletter
  % The setting for indentations:
  \def\progindent@indentation{\quad}

  % The escaped alignment tab and break:
  \def\progindent@firstalign{&}
  \def\progindent@breakandalign{\\&}

  % The so-called hop trick:
  \def\progindent@then#1\else#2\fi{\fi#1}

  % The tokens for the progindent DSL:
  \def\br{\progindent@br@dummy}
  \def\deepen{\progindent@deepen@dummy}
  \def\finished{\progindent@finished@dummy}

  % Forms a region for the progindent DSL:
  \newcommand\progindent[1]{%
    \progindent@firstalign
    \progindent@main{}{#1}%
  }
  \def\progindent@main#1#2{%
    % #1 : current indentation
    % #2 : contents
    \progindent@iterA{#1}#2\control\finished\progindent@end
  }
  \def\progindent@iterA#1#2\control#3#4\progindent@end{%
    % #1 : current indentation
    % #2 : contents before the first \control
    % #3 : the token immediately after the first \control
    %      (expected to be either \deepen, \br, or \finished)
    % #4 : contents after #3
    #2%
    \ifx\finished#3\else
      \progindent@iterB{#1}{#3}{#4}%
    \fi
  }
  \def\progindent@iterB#1#2#3{%
    % #1 : current indentation
    % #2 : the token immediately after the first \control
    %      (expected to be either \deepen, \br, or \finished)
    % #3 : contents after #2
    \ifx\br#2%
      \progindent@br{#1}#3\progindent@end
    \else
      \progindent@iterC{#1}{#2}{#3}%
    \fi
  }
  \def\progindent@iterC#1#2#3{%
    % #1 : current indentation
    % #2 : the token immediately after the first \control
    %      (expected to be either \deepen, \br, or \finished)
    % #3 : contents after #2
    \ifx\deepen#2%
      \progindent@deepen{#1}#3\progindent@end
    \else
      % Emits an error:
      \errmessage{Invalid token after \string\control.}%
    \fi
  }
  \def\progindent@br#1#2#3\progindent@end{%
    % #1 : current indentation
    % #2 : an argument of \br (i.e. ignored punctuation)
    % #3 : subsequent contents
    \progindent@breakandalign#1%
    \progindent@iterA{#1}#3\progindent@end
  }
  \def\progindent@deepen#1#2#3\progindent@end{%
    % #1 : current indentation
    % #2 : an argument of \deepen (i.e. contents to deepen)
    % #3 : subsequent contents
    \progindent@main{#1\progindent@indentation}{#2}%
    \progindent@iterA{#1}#3\progindent@end
  }
  % The definiton of the expansion of \control outside the \progindent.
  % Ignores the effect of \br and \deepen:
  \newcommand\control[1]{%
    % #1 : the token immediately after the \control
    \ifx\br#1%
    \else
      \progindent@control{#1}%
    \fi
  }
  \def\progindent@control#1{%
    % #1 : the token immediately after the \control
    \ifx\deepen#1\progindent@then
      \progindent@ignoredeepen
    \else
      % Emits an error:
      \errmessage{Invalid token after \string\control.}%
    \fi
  }
  \def\progindent@ignoredeepen#1{%
    % #1 : the argument of \deepen
    #1%
  }
\makeatother


==> proglangtools/proginfer.tex <==
\makeatletter
  % Requires `bussproofs`

  \def\proginfer@unique{\proginfer@unique@dummy}
  \def\proginfer@ifempty#1#2#3{%
    \ifx\proginfer@unique#1\proginfer@unique#2\else#3\fi
  }
  \newcommand\rulename[1]{\textsc{#1}}
  % Usage:
  % - \derive{〈Hypotheses〉}{〈Conclusion〉}
  % - \derive[〈RuleName〉]{〈Hypotheses〉}{〈Conclusion〉}
  % Typesets an inference rule.
  % The format of arguments is the same as that of `\infrule` of `bcprules.sty`,
  % i.e., hypotheses are separated by `\andalso` or `\\`:
  \newcommand\derive[3][]{%
    \(\displaystyle
      \frac{\begin{array}{@{}c@{}}#2\end{array}}{\begin{array}{@{}c@{}}#3\end{array}}
    \)\proginfer@ifempty{#1}{}{\hbox{\,{\scriptsize\rulename{#1}}}}%
  }
  \newcommand\andalso{\qquad}
  % A variant version of `\derive` that can be nested.
  % `\\` cannot be used in hypotheses, however:
  \newcommand\infer[3][]{%
    \proginfer@infer[#1]{#2}{#3}%
    %\bottomAlignProof %(a vertical alignment option)
    \DisplayProof
  }
  \newcommand\proginfer@infer[3][]{%
    \proginfer@inferiter#2\andalso\proginfer@end{1}{#3}{%
      \proginfer@ifempty{#1}{}{\RightLabel{\scriptsize\rulename{#1}}}%
    }%
  }
  \def\proginfer@inferiter#1\andalso#2\proginfer@end#3#4#5{%
    % - #1: one of the formulas for the hypotheses.
    % - #2: the rest hypotheses.
    % - #3: an index for hypothesis #1 (one-based).
    % - #4: a formula for the conclusion.
    % - #5: a RightLabel spec if necessary, or empty otherwise.
    \proginfer@buildhypo{#1}%
    \ifcase#3\relax
      % #3 == 0 cannot happen.
    \or
      \proginfer@ifempty{#2}{%
        #5\UnaryInfC{\(#4\)}
      }{%
        \proginfer@inferiter#2\proginfer@end{2}{#4}{#5}%
      }%
    \or
      \proginfer@ifempty{#2}{
        #5\BinaryInfC{\(#4\)}%
      }{%
        \proginfer@inferiter#2\proginfer@end{3}{#4}{#5}%
      }%
    \or
      \proginfer@ifempty{#2}{%
        #5\TrinaryInfC{\(#4\)}%
      }{%
        \proginfer@inferiter#2\proginfer@end{4}{#4}{#5}%
      }%
    \or
      \proginfer@ifempty{#2}{
        #5\QuaternaryInfC{\(#4\)}%
      }{%
        \proginfer@inferiter#2\proginfer@end{5}{#4}{#5}%
      }%
    \or
      \proginfer@ifempty{#2}{
        #5\QuinaryInfC{\(#4\)}%
      }{%
        \proginfer@inferiter#2\proginfer@end{6}{#4}{#5}%
      }%
    \else
      \errmessage{More than five hypotheses.}%
    \fi
  }
  % If the first token of `#1` is `\infer`, then this command returns `#1` as it is,
  % or wrap `#1` with `\AxiomC` otherwise.
  \def\proginfer@buildhypo#1{%
    \proginfer@ifempty{#1}{%
      \AxiomC{}%
    }{%
      \expandafter\ifx\proginfer@firsttoken#1\proginfer@end\infer
        \proginfer@chopinfer#1%
      \else
        \AxiomC{\(#1\)}%
      \fi
    }%
  }
  % Replaces the leftmost `\infer` with `\proginfer@infer` with spaces ignored by `#1`:
  \def\proginfer@chopinfer#1\infer{\proginfer@infer}
  \def\proginfer@firsttoken#1#2\proginfer@end{#1}
\makeatother

